Challenging Common Assumptions about Catastrophic Forgetting

Building learning agents that can progressively learn and accumulate knowledge is the core goal of the continual learning (CL) research field. Unfortunately, training a model on new data usually compromises the performance on past data. In the CL literature, this effect is referred to as catastrophic forgetting (CF). CF has been largely studied, and a plethora of methods have been proposed to address it on short sequences of non-overlapping tasks. In such setups, CF always leads to a quick and significant drop in performance in past tasks. Nevertheless, despite CF, recent work showed that SGD training on linear models accumulates knowledge in a CL regression setup. This phenomenon becomes especially visible when tasks reoccur. We might then wonder if DNNs trained with SGD or any standard gradient-based optimization accumulate knowledge in such a way. Such phenomena would have interesting consequences for applying DNNs to real continual scenarios. Indeed, standard gradient-based optimization methods are significantly less computationally expensive than existing CL algorithms. In this paper, we study the progressive knowledge accumulation (KA) in DNNs trained with gradient-based algorithms in long sequences of tasks with data re-occurrence. We propose a new framework, SCoLe (Scaling Continual Learning), to investigate KA and discover that catastrophic forgetting has a limited effect on DNNs trained with SGD. When trained on long sequences with data sparsely re-occurring, the overall accuracy improves, which might be counter-intuitive given the CF phenomenon. We empirically investigate KA in DNNs under various data occurrence frequencies and propose simple and scalable strategies to increase knowledge accumulation in DNNs.

==> Algo/scole.tex <==

\begin{algorithm}[H]
\caption{{\bf Scole Scenario}. {\footnotesize Controling reoccurence and non-stationnarity with Scole.}}
\begin{algorithmic}[1]
  \State \textbf{Input:} \textit{total Number of classes $N$, classes per task $C$, number of epochs $E$, $\mathcal{P}$}
    \For{t in nb\_tasks}
        \State Samples $C$ classes without replacement with $\mathcal{P}$: $classes \sim \mathcal{P}(N)$ %\Comment{{\tiny Samples $C$ classes without replacement with $\mathcal{P}$}}
        
        \While {epochs}
        \State Sample data from classes $x_t, y_t \sim \mathcal{D}[classes]$
        \State Get loss $\mathcal{L}(\theta_{t-1}(x_t), y_t)$
        \State Update $\theta$
        \EndWhile
        \State eval on whole test data $eval(\theta_t(\mathcal{D_{te}}))$
    \EndFor
\end{algorithmic}
\label{alg:reservoir}
\end{algorithm}

==> Tables/table_influence.tex <==


\begin{table}
\centering
\begin{tabular}{|lp{2cm}p{2cm}p{2cm}p{2cm}p{2cm}}
\toprule
\textbf{Parameters} & N $\uparrow$ & C $\uparrow$ & $\mathcal{P}$ Entropy $\uparrow$ & epoch/iterations per task $\uparrow$ & Data Augmentation\\ \midrule
Influence & $\uparrow$ & $\downarrow$ & $\downarrow$ & $\uparrow$ & $\uparrow$ \\ \bottomrule
\end{tabular}
\end{table}
